A Point-Based Approach to Efficient LiDAR Multi-Task Perception

Multi-task networks can potentially improve performance and computational efficiency compared to single-task networks, facilitating online deployment. However, current multi-task architectures in point cloud perception combine multiple task-specific point cloud representations, each requiring a separate feature encoder and making the network structures bulky and slow. We propose PAttFormer, an efficient multi-task architecture for joint semantic segmentation and object detection in point clouds that only relies on a point-based representation. The network builds on transformer-based feature encoders using neighborhood attention and grid-pooling and a query-based detection decoder using a novel 3D deformable-attention detection head design. Unlike other LiDAR-based multi-task architectures, our proposed PAttFormer does not require separate feature encoders for multiple task-specific point cloud representations, resulting in a network that is 3x smaller and 1.4x faster while achieving competitive performance on the nuScenes and KITTI benchmarks for autonomous driving perception. Our extensive evaluations show substantial gains from multi-task learning, improving LiDAR semantic segmentation by +1.7% in mIou and 3D object detection by +1.7% in mAP on the nuScenes benchmark compared to the single-task models.

==> alg/grid_query.tex <==
\begin{algorithm}
\caption{An algorithm with caption}\label{alg:grid_query}
\KwData{query points $\mathbf{q}$, pointcloud points $\mathbf{p}_i \in \mathbf{P}$, max group distance $d_{max}$, max group size $M$, max search cells $K_{max}$}
\KwResult{$M$ neighbor point indices $\mathbf{m}$, relative positions of neighbors to query point $\Delta \mathbf{P} \in \mathcal{R}^{3 \times M}$}
$y \gets 1$\;
$X \gets x$\;
$N \gets n$\;
\While{$N \neq 0$}{
    $d_{q,p_i} = |q_x - p_{i,x}| + |q_y - p_{i,y}| + |q_z - p_{i,z}|$\;
  \eIf{$d_{q,p_i} < \sqrt{d_{max}}$}{
    $m \gets i$\;
  }
  \# Check for termination criterion
  \If{len$(\mathbf{m}) \geq M$ or $(k \geq K)$}{
    return $\mathbf{m}$ \;
  }
}
\end{algorithm}

==> tab/detection/nuscenes_val.tex <==
\begin{table*}[]
\scriptsize
\centering
\caption{Detection results on the nuScenes val split.}
\label{tab:nus_det_val}
\begin{tabular}{lllllllll} \toprule
                      &               & mAP  & NDS  & $mAP_{c}$ & $mAP_{f}$    & \# M Params & \multicolumn{2}{l}{Runtime {[}ms{]}} \\
                      &               &      &      & >30m      & 30> x <50m &             & Backbone          & Decoder          \\ \midrule
SphereFormer          &               & 68.5 & 72.8 &           &            &             &                   &                  \\
DeformFormer3D        & DDETR         & 65.5 & 70.7 &           &            &             &                   & 14.8             \\
FocalFormer3D         & Focal Decoder & 66.4 & 70.9 &           &            &             & 91                & 18               \\
SparseConv            & DDETR         & 62.8 & 68.5 & 66.9      & 52.3       &             & 94                & 13               \\
SphereFormer & DDETR         & 64.0 & 68.5 & 68.5      & 55.2       & 32.3        & 123               & 13               \\ \midrule
Patt                  & DDETR         & 65.0 & 70.3 & 69.5      & 57.9       & 27.8        & 104               & 13               \\
Patt-only             & DDETR         & 64.7 & 70.2 & 69.0      & 57.2       & 21.5        & 80                & 13               \\
Patt-only             & 3D SSD        & 55.4 & 64.1 &           &            & 18.2        & 80                & 24     \\ \bottomrule          
\end{tabular}
\end{table*}




\begin{table}[]
\scriptsize
\centering
\caption{Effect of weight decay hyper-parameter on detection performance.}
\label{tab:my-table}
\begin{tabular}{lllll} \toprule
Backbone & Decoder head    & Weight decay & mAP  & NDS  \\ \midrule
Patt     & Deformable DETR & 1.00E-04     & 63.0 & 69.0 \\
         &                 & 5.00E-03     & 65.0 & 70.3 \\
         &                 & 1.00E-03     & 48.9 & 54.6 \\
         &                 & 1.00E-02     & 32.7 & 38.1 \\ \bottomrule
\end{tabular}
\end{table}

==> tab/nuscenes.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{Comparison with state-of-the-art methods on the test sets of three nuScenes benchmarks. A single PAtt model is used to generate predictions for all three tasks.}
\label{tab:nuscenes_test}
\begin{tabular}{llllllll}
                              & Methods           & Reference   & mloU & mAP  & ND S & PQ   & mloU \\
\multirow{9}{*}{Segmentation} & PolarNet          & CVPR 020    & 69.8 &      &      &      &      \\
                              & PolarStream       & Neur1PS 021 & 73.4 &      &      &      &      \\
                              & JS3C-Net          & AAAI 2021   & 73.4 &      &      &      &      \\
                              & AMVNet            & IJCAIW 2021 & 77.3 &      &      &      &      \\
                              & SPVNAS            & ECCV 020    & 77.4 &      &      &      &      \\
                              & Cylinder3D++      & CVPR 021b   & 77.9 &      &      &      &      \\
                              & AF2S3Net          & CVPR 021    & 78.3 &      &      &      &      \\
                              & DRINet++          & arXiv 02 la & 80.4 &      &      &      &      \\
                              & SPVCNN++          & ECCV 2020   & 81.1 &      &      &      &      \\
\multirow{9}{*}{Detection}    & Cylinder3D        & TPAMI 021a  &      & 50.6 & 61.6 &      &      \\
                              & CBGS              & arXiv 019   &      & 52.8 & 63.3 &      &      \\
                              & CenterPoint       & CVPR 021    &      & 58   & 65.5 &      &      \\
                              & HotSpotNet        & ECCV 2020   &      & 59.3 & 66   &      &      \\
                              & Object DGCNN      & Neur1PS 021 &      & 58.7 & 66.1 &      &      \\
                              & AFDetV2           & AAAI 022    &      & 62.4 & 68.5 &      &      \\
                              & Focals Conv       & CVPR 022b   &      & 63.8 & 70   &      &      \\
                              & TransFusion-L     & CVPR 022    &      & 65.5 & 70.2 &      &      \\
                              & LargeKerne13D     & arXiv 022c  &      & 65.3 & 70.5 &      &      \\
\multirow{4}{*}{Panoptic}     & EfficientLPS      & T-RO 021    &      &      &      & 62.4 & 66.7 \\
                              & Panoptic-PolarNet & CVPR 021    &      &      &      & 63.6 & 67   \\
                              & SPVCNN++          & ECCV 2020   &      &      &      & 79.1 & 80.3 \\
                              & Panoptic-PHNet    & CVPR 022a   &      &      &      & 80.1 & 80.2 \\
                              & LidarMultiNet     & Ours        & 81.4 & 67   & 71.6 & 81.4 &     
\end{tabular}
\end{table}

==> tab/segmentation/kitti.tex <==
single task performancec.
\begin{tabular}{cccccccccccccccccccccc}
Approach & mean IoU & mean accuracy & car & bicycle & motorcycle & truck & other-vehicle & person & bicyclist & motorcyclist & road & parking & sidewalk & other-ground & building & fence & vegetation & trunk & terrain & pole & traffic-sign \\
Anonymous & 67.1 & 90.7 & 96.8 & 59.5 & 56.3 & 53.1 & 54.6 & 77.3 & 81.4 & 17.4 & 88.9 & 66.5 & 74.1 & 31.1 & 92.0 & 67.9 & 84.3 & 73.8 & 68.4 & 62.4 & 68.4 \\
\end{table}

==> tab/task_affinity.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{Inter-task affinity measures for multi-task architectures.}
\label{tab:task_affinity}
\begin{tabular}{@{}llll@{}}
\toprule
Inter-task affinity & \begin{tabular}[c]{@{}l@{}}ResNet \\ (vision)\end{tabular} & \begin{tabular}[c]{@{}l@{}}MinkUCP\\ (lidar)\end{tabular} & \begin{tabular}[c]{@{}l@{}}PAttFormer \\ (lidar)\end{tabular} \\ \midrule
Det $\rightarrow$ Seg          & 0.126                                                      & 0.001                                                            & 0.153                                                         \\
Seg $\rightarrow$ Det          & 0.092                                                      & 0.003                                                            & 0.121                                                         \\ \bottomrule
\end{tabular}
\vspace{-0.3cm}
\end{table}
